The economic impact of weather and climate

I propose a new conceptual framework to disentangle the impacts of weather and climate on economic activity and growth: A stochastic frontier model with climate in the production frontier and weather shocks as a source of inefficiency. I test it on a sample of 160 countries over the period 1950-2014. Temperature and rainfall determine production possibilities in both rich and poor countries; positively in cold countries and negatively in hot ones. Weather anomalies reduce inefficiency in rich countries but increase inefficiency in poor and hot countries; and more so in countries with low weather variability. The climate effect is larger that the weather effect.

==> Table2a.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Baseline results.Dependent variable: ln(output per worker).\label{tab:base}}
\scriptsize \begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
frontier            &                     &                     &                     &                     &                     &                     \\
$\ln(k)$            &       0.613\sym{***}&       0.613\sym{***}&       0.616\sym{***}&       0.613\sym{***}&       0.619\sym{***}&       0.622\sym{***}\\
                    &     (76.09)         &     (75.31)         &     (74.57)         &     (74.72)         &     (76.00)         &     (75.65)         \\
[1em]
$T$                 &       0.189\sym{***}&       0.183\sym{***}&       0.181\sym{***}&       0.183\sym{***}&       0.207\sym{***}&       0.205\sym{***}\\
                    &      (8.02)         &      (7.70)         &      (7.63)         &      (7.72)         &      (8.61)         &      (8.51)         \\
[1em]
$T^2$               &    -0.00547\sym{***}&    -0.00556\sym{***}&    -0.00563\sym{***}&    -0.00568\sym{***}&    -0.00488\sym{***}&    -0.00486\sym{***}\\
                    &     (-7.91)         &     (-8.18)         &     (-8.20)         &     (-8.45)         &     (-6.72)         &     (-6.61)         \\
[1em]
$R$                 &    0.000544         &     0.00725         &     0.00689         &     0.00987         &      0.0882\sym{***}&      0.0835\sym{***}\\
                    &      (0.05)         &      (0.64)         &      (0.61)         &      (0.87)         &      (4.54)         &      (4.36)         \\
[1em]
$R^2$               &  -0.0000150         &   -0.000542         &   -0.000525         &   -0.000599         &    0.000347         &    0.000418         \\
                    &     (-0.04)         &     (-1.37)         &     (-1.33)         &     (-1.56)         &      (0.90)         &      (1.06)         \\
[1em]
Trend               &     0.00329\sym{***}&     0.00328\sym{***}&     0.00336\sym{***}&     0.00338\sym{***}&     0.00316\sym{***}&     0.00314\sym{***}\\
                    &     (11.14)         &     (11.16)         &     (11.19)         &     (11.57)         &     (10.67)         &     (10.30)         \\
[1em]
$P \times T$        &                     &       0.329\sym{*}  &       0.325\sym{*}  &       0.371\sym{*}  &       1.011\sym{***}&       0.954\sym{***}\\
                    &                     &      (2.19)         &      (2.21)         &      (2.46)         &      (4.23)         &      (4.06)         \\
[1em]
$P \times T^2$      &                     &    -0.00540         &    -0.00513         &    -0.00621\sym{*}  &     -0.0163\sym{***}&     -0.0150\sym{***}\\
                    &                     &     (-1.74)         &     (-1.70)         &     (-2.01)         &     (-3.86)         &     (-3.64)         \\
[1em]
$P \times R$        &                     &      0.0131         &      0.0244         &      0.0181         &       0.459\sym{***}&       0.454\sym{***}\\
                    &                     &      (0.36)         &      (0.68)         &      (0.51)         &      (3.61)         &      (3.55)         \\
[1em]
$P \times R^2$      &                     &    0.000803         &    0.000540         &    0.000638         &    -0.00192         &    -0.00205         \\
                    &                     &      (0.83)         &      (0.56)         &      (0.67)         &     (-1.84)         &     (-1.94)         \\
[1em]
$T \times R$        &                     &                     &                     &                     &    -0.00495\sym{***}&    -0.00483\sym{***}\\
                    &                     &                     &                     &                     &     (-5.96)         &     (-5.91)         \\
[1em]
$P \times T \times R$&                     &                     &                     &                     &     -0.0140\sym{**} &     -0.0135\sym{**} \\
                    &                     &                     &                     &                     &     (-3.17)         &     (-3.05)         \\
\hline
usigmas             &                     &                     &                     &                     &                     &                     \\
$ |z(T)| $          &      0.0246         &      0.0226         &     -0.0531         &     -0.0622         &     -0.0642         &     -0.0536         \\
                    &      (0.75)         &      (0.68)         &     (-1.48)         &     (-1.63)         &     (-1.68)         &     (-1.50)         \\
[1em]
$ |z(R)| $          &     0.00243         &     0.00342         &     -0.0859\sym{*}  &      -0.109\sym{**} &      -0.109\sym{**} &     -0.0855\sym{*}  \\
                    &      (0.07)         &      (0.09)         &     (-2.10)         &     (-2.72)         &     (-2.72)         &     (-2.09)         \\
[1em]
$ P \times |z(T)| $ &                     &                     &       0.193\sym{***}&       0.183\sym{**} &       0.181\sym{**} &       0.192\sym{***}\\
                    &                     &                     &      (3.31)         &      (3.08)         &      (3.07)         &      (3.33)         \\
[1em]
$ P \times |z(R)| $ &                     &                     &       0.272\sym{***}&       0.257\sym{***}&       0.252\sym{***}&       0.267\sym{***}\\
                    &                     &                     &      (4.14)         &      (3.78)         &      (3.73)         &      (4.11)         \\
[1em]
$ H \times |z(R)| $ &                     &                     &                     &      0.0709         &      0.0805         &                     \\
                    &                     &                     &                     &      (1.20)         &      (1.37)         &                     \\
[1em]
$ H \times |z(R)| $ &                     &                     &                     &      0.0981         &       0.101         &                     \\
                    &                     &                     &                     &      (1.37)         &      (1.42)         &                     \\
\hline
Observations        &        7753         &        7753         &        7753         &        7753         &        7753         &        7753         \\
logl                &      2041.7         &      2049.3         &      2106.0         &      2112.0         &      2130.7         &      2123.7         \\
eff                 &       0.814         &       0.814         &       0.816         &       0.814         &       0.814         &       0.814         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table}


==> TableTrend.tex <==
{\scriptsize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{longtable}{l*{6}{c}}
\caption{Robustness. Dependent variable: ln(output per worker).\label{tab:trend}}\\
\hline\hline\endfirsthead\hline\endhead\hline\endfoot\endlastfoot
                    &\multicolumn{1}{c}{no trend}&\multicolumn{1}{c}{linear}&\multicolumn{1}{c}{quadratic}&\multicolumn{1}{c}{cubic}&\multicolumn{1}{c}{split}&\multicolumn{1}{c}{first diff.}\\
\hline
\multicolumn{7}{c}{frontier} \\
$\ln(k)$            &       0.692\sym{***}&       0.631\sym{***}&       0.630\sym{***}&       0.619\sym{***}&       0.622\sym{***}& 0.625\sym{***}                    \\
                    &    (117.70)         &     (77.76)         &     (77.91)         &     (74.82)         &     (75.62)         &      (21.21)               \\
[1em]
$T$                 &       0.254\sym{***}&       0.226\sym{***}&       0.232\sym{***}&       0.164\sym{***}&       0.218\sym{***}&  0.0909\sym{*}                   \\
                    &      (9.46)         &      (8.58)         &      (7.71)         &      (6.11)         &      (8.08)         &    (2.17)                 \\
[1em]
$T^2$               &    -0.00244\sym{**} &    -0.00457\sym{***}&    -0.00463\sym{***}&    -0.00440\sym{***}&    -0.00392\sym{***}&  -0.00233                   \\
                    &     (-3.10)         &     (-5.42)         &     (-5.31)         &     (-6.01)         &     (-4.65)         &    (-1.60)                 \\
[1em]
$R$                 &       0.233\sym{***}&       0.244\sym{***}&       0.243\sym{***}&       0.253\sym{***}&       0.258\sym{***}&  0.0408                   \\
                    &      (6.03)         &      (6.89)         &      (6.82)         &      (7.24)         &      (7.36)         &    (1.78)                 \\
[1em]
$R^2$               &     0.00516\sym{**} &     0.00570\sym{**} &     0.00574\sym{**} &     0.00459\sym{*}  &     0.00685\sym{**} &  0.000405                   \\
                    &      (2.67)         &      (2.85)         &      (2.83)         &      (2.45)         &      (3.18)         &     (0.66)                \\
[1em]
$T \times R$        &     -0.0185\sym{***}&     -0.0199\sym{***}&     -0.0199\sym{***}&     -0.0200\sym{***}&     -0.0221\sym{***}&    -0.00209                  \\
                    &     (-6.82)         &     (-8.45)         &     (-8.44)         &     (-8.75)         &     (-9.00)         &     (-1.79)                \\
[1em]
$P \times R$        &      -0.138\sym{*}  &      -0.146\sym{**} &      -0.146\sym{**} &      -0.197\sym{***}&      -0.212\sym{***}&  -0.119\sym{*}                   \\
                    &     (-2.47)         &     (-3.05)         &     (-3.05)         &     (-4.82)         &     (-4.55)         &   (-2.11)                  \\
[1em]
$P \times R^2$      &    -0.00438\sym{*}  &    -0.00614\sym{**} &    -0.00617\sym{**} &    -0.00461\sym{*}  &    -0.00664\sym{**} &   -0.00121                  \\
                    &     (-2.22)         &     (-2.96)         &     (-2.95)         &     (-2.41)         &     (-2.99)         &   (-1.25)                  \\
[1em]
$P \times T \times R$&      0.0135\sym{***}&      0.0172\sym{***}&      0.0172\sym{***}&      0.0183\sym{***}&      0.0202\sym{***}&   0.00594\sym{**}                  \\
                    &      (4.45)         &      (6.50)         &      (6.50)         &      (7.42)         &      (7.57)         &      (2.68)               \\
[1em]
\hline
\multicolumn{7}{c}{inefficiency}  \\
$ |z(T)| $          &      -0.216\sym{***}&      -0.202\sym{***}&      -0.203\sym{***}&      -0.207\sym{***}&      -0.187\sym{***}&      -0.118         \\
                    &     (-3.76)         &     (-3.54)         &     (-3.53)         &     (-3.48)         &     (-3.33)         &     (-1.28)         \\
[1em]
$ |z(R)| $          &      -0.215\sym{***}&      -0.266\sym{***}&      -0.268\sym{***}&      -0.299\sym{***}&      -0.282\sym{***}&      -0.106         \\
                    &     (-3.75)         &     (-4.53)         &     (-4.50)         &     (-4.74)         &     (-4.88)         &     (-0.82)         \\
[1em]
$ P \times |z(T)| $ &       0.257\sym{***}&       0.259\sym{***}&       0.260\sym{***}&       0.236\sym{***}&       0.228\sym{***}&       0.215         \\
                    &      (4.03)         &      (4.05)         &      (4.04)         &      (3.46)         &      (3.62)         &      (1.68)         \\
[1em]
$ P \times |z(R)| $ &       0.238\sym{***}&       0.282\sym{***}&       0.285\sym{***}&       0.318\sym{***}&       0.296\sym{***}&       0.345\sym{*}  \\
                    &      (3.41)         &      (4.01)         &      (3.98)         &      (4.13)         &      (4.35)         &      (2.05)         \\
[1em]
$ H \times |z(T)| $ &       0.189\sym{**} &       0.229\sym{***}&       0.229\sym{***}&       0.238\sym{***}&       0.246\sym{***}&       0.135         \\
                    &      (2.99)         &      (3.49)         &      (3.48)         &      (3.50)         &      (3.84)         &      (1.00)         \\
[1em]
$ H \times |z(R)| $ &       0.183\sym{**} &       0.231\sym{**} &       0.232\sym{**} &       0.245\sym{***}&       0.259\sym{***}&     -0.0492         \\
                    &      (2.70)         &      (3.25)         &      (3.25)         &      (3.33)         &      (3.73)         &     (-0.28)         \\
[1em]
$ L.|z(T)| $            &                     &                     &                     &                     &                     &       0.124         \\
                    &                     &                     &                     &                     &                     &      (1.38)         \\
[1em]
$ L.|z(R)| $             &                     &                     &                     &                     &                     &     -0.0305         \\
                    &                     &                     &                     &                     &                     &     (-0.29)         \\
[1em]
$ P \times L.|z(T)| $           &                     &                     &                     &                     &                     &      -0.201         \\
                    &                     &                     &                     &                     &                     &     (-1.75)         \\
[1em]
$ P \times L.|z(R)| $           &                     &                     &                     &                     &                     &      0.0307         \\
                    &                     &                     &                     &                     &                     &      (0.91)         \\
[1em]
$ H \times L.|z(T)| $            &                     &                     &                     &                     &                     &     -0.0466         \\
                    &                     &                     &                     &                     &                     &     (-0.39)         \\
[1em]
$ H \times L.|z(R)| $            &                     &                     &                     &                     &                     &      0.0387         \\
                    &                     &                     &                     &                     &                     &      (0.27)         \\
\hline
Observations        &        7753         &        7753         &        7753         &        7753         &        7753         &        7591         \\
LpL                &      2439.0         &      2556.5         &      2556.7         &      2775.4         &      2585.7         &     11337.1         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{longtable}
}

